U-Net Fixed-Point Quantization for Medical Image Segmentation

Model quantization is leveraged to reduce the memory consumption and the computation time of deep neural networks. This is achieved by representing weights and activations with a lower bit resolution when compared to their high precision floating point counterparts. The suitable level of quantization is directly related to the model performance. Lowering the quantization precision (e.g. 2 bits), reduces the amount of memory required to store model parameters and the amount of logic required to implement computational blocks, which contributes to reducing the power consumption of the entire system. These benefits typically come at the cost of reduced accuracy. The main challenge is to quantize a network as much as possible, while maintaining the performance accuracy. In this work, we present a quantization method for the U-Net architecture, a popular model in medical image segmentation. We then apply our quantization algorithm to three datasets: (1) the Spinal Cord Gray Matter Segmentation (GM), (2) the ISBI challenge for segmentation of neuronal structures in Electron Microscopic (EM), and (3) the public National Institute of Health (NIH) dataset for pancreas segmentation in abdominal CT scans. The reported results demonstrate that with only 4 bits for weights and 6 bits for activations, we obtain 8 fold reduction in memory requirements while loosing only 2.21%, 0.57% and 2.09% dice overlap score for EM, GM and NIH datasets respectively. Our fixed point quantization provides a flexible trade off between accuracy and memory requirement which is not provided by previous quantization methods for U-Net such as TernaryNet.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> references_back.tex <==
%
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%
% \bibliographystyle{splncs04}
% \bibliography{mybibliography}
%

\begin{thebibliography}{10}

\bibitem{abdelouahab:hal-01695375}
Kamel Abdelouahab, Maxime Pelcat, Fran{\c c}ois Berry, and Jocelyn S{\'e}rot.
\newblock {Accelerating CNN inference on FPGAs: A Survey}.
\newblock working paper or preprint, March 2018.

\bibitem{badrinarayanan2015segnet}
V.~{Badrinarayanan}, A.~{Kendall}, and R.~{Cipolla}.
\newblock Segnet: A deep convolutional encoder-decoder architecture for image
  segmentation.
\newblock {\em IEEE Transactions on Pattern Analysis and Machine Intelligence},
  39(12):2481--2495, Dec 2017.

\bibitem{BoltzmanQuant}
Wolfgang Balzer, Masanobu Takahashi, Jun Ohta, and Kazuo Kyuma.
\newblock Weight quantization in boltzmann machines.
\newblock {\em Neural Networks}, 4, 1991.

\bibitem{bulat2018hierarchical}
Adrian Bulat and Georgios Tzimiropoulos.
\newblock Hierarchical binary cnns for landmark localization with limited
  resources.
\newblock {\em IEEE Transactions on Pattern Analysis and Machine Intelligence},
  2018.

\bibitem{NIPS20155647}
Matthieu Courbariaux, Yoshua Bengio, and Jean-Pierre David.
\newblock Binaryconnect: Training deep neural networks with binary weights
  during propagations.
\newblock In C.Cortes, N.D. Lawrence, D.D. Lee, M.Sugiyama, and R.Garnett, editors, {\em Advances in Neural Information Processing Systems 28}, pages 3123--3131. Curran Associates, Inc., 2015.

\bibitem{cciccek20163d}
{\"O}zg{\"u}n {\c{C}}i{\c{c}}ek, Ahmed Abdulkadir, Soeren~S Lienkamp, Thomas
  Brox, and Olaf Ronneberger.
\newblock 3d u-net: learning dense volumetric segmentation from sparse
  annotation.
\newblock In {\em International Conference on Medical Image Computing and
  Computer-Assisted Intervention}, pages 424--432. Springer, 2016.


\bibitem{DBLP:journals/corr/abs-1708-01001}
Yinpeng Dong, Renkun Ni, Jianguo Li, Yurong Chen, Jun Zhu, and Hang Su.
\newblock Learning accurate low-bit deep neural networks with stochastic
  quantization.
\newblock {\em CoRR}, abs/1708.01001, 2017.

\bibitem{fiesler1990quantization}
Emile Fiesler, Choudry Amar, and H~John Caulfield.
\newblock Weight discretization paradigm for optical neural networks.
\newblock pages 164--173, 1990.

\bibitem{fowers2018configurable}
Jeremy Fowers, Kalin Ovtcharov, Michael Papamichael, Todd Massengill, Ming Liu,
  Daniel Lo, Shlomi Alkalay, Michael Haselman, Logan Adams, Mahdi Ghandi,
  et~al.
\newblock A configurable cloud-scale dnn processor for real-time ai.
\newblock In {\em Proceedings of the 45th Annual International Symposium on
  Computer Architecture}, pages 1--14. IEEE Press, 2018.

\bibitem{DBLP:journals/corr/abs-1808-04752}
Yunhui Guo.
\newblock A survey on methods and theories of quantized neural networks.
\newblock {\em CoRR}, abs/1808.04752, 2018.

\bibitem{Gupta:2015:DLL:3045118.3045303}
Suyog Gupta, Ankur Agrawal, Kailash Gopalakrishnan, and Pritish Narayanan.
\newblock Deep learning with limited numerical precision.
\newblock In {\em Proceedings of the 32Nd International Conference on
  International Conference on Machine Learning - Volume 37}, ICML'15, pages
  1737--1746. JMLR.org, 2015.

\bibitem{STECoursera}
Geoffrey Hinton, Nitsh Srivastava, and Kevin Swersky.
\newblock Neural networks for machine learning, video lectures.
\newblock {\em Coursera}, 2012.

\bibitem{hinton2012improving}
Geoffrey~E Hinton, Nitish Srivastava, Alex Krizhevsky, Ilya Sutskever, and
  Ruslan~R Salakhutdinov.
\newblock Improving neural networks by preventing co-adaptation of feature
  detectors.
\newblock {\em arXiv preprint arXiv:1207.0580}, 2012.

\bibitem{honari2016recombinator}
Sina Honari, Jason Yosinski, Pascal Vincent, and Christopher Pal.
\newblock Recombinator networks: Learning coarse-to-fine feature aggregation.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 5743--5752, 2016.

\bibitem{IEEE:ISSCC}
Mark Horowitz.
\newblock Computing’s energy problem (and what we can do about it).
\newblock {\em Interational Solid State Circuits Conference}, 2014.

\bibitem{DBLP:journals/corr/HubaraCSEB16}
Itay Hubara, Matthieu Courbariaux, Daniel Soudry, Ran El-Yaniv, and Yoshua
  Bengio.
\newblock Quantized neural networks: Training neural networks with low
  precision weights and activations.
\newblock {\em Journal of Machine Learning Research}, 18(187):1--30, 2018.

\bibitem{isola2017image}
Phillip Isola, Jun-Yan Zhu, Tinghui Zhou, and Alexei~A. Efros.
\newblock Image-to-image translation with conditional adversarial networks.
\newblock In {\em The IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}, July 2017.

\bibitem{jouppi2017datacenter}
Norman~P Jouppi, Cliff Young, Nishant Patil, David Patterson, Gaurav Agrawal,
  Raminder Bajwa, Sarah Bates, Suresh Bhatia, Nan Boden, Al~Borchers, et~al.
\newblock In-datacenter performance analysis of a tensor processing unit.
\newblock In {\em Computer Architecture (ISCA), 2017 ACM/IEEE 44th Annual
  International Symposium on}, pages 1--12. IEEE, 2017.

\bibitem{CIFAR10}
Alex Krizhevsky, Vinod Nair, and Geoffrey Hinton.
\newblock Cifar-10 (canadian institute for advanced research).

\bibitem{DBLP:journals/corr/LiL16}
Fengfu Li and Bin Liu.
\newblock Ternary weight networks.
\newblock {\em CoRR}, abs/1605.04711, 2016.

\bibitem{DBLP:journals/corr/LinTA15}
Darryl Lin, Sachin Talathi, and Sreekanth Annapureddy.
\newblock Fixed point quantization of deep convolutional networks.
\newblock In Maria~Florina Balcan and Kilian~Q. Weinberger, editors, {\em
  Proceedings of The 33rd International Conference on Machine Learning},
  volume~48 of {\em Proceedings of Machine Learning Research}, pages
  2849--2858, New York, New York, USA, 20--22 Jun 2016. PMLR.

\bibitem{litjens2017survey}
Geert Litjens, Thijs Kooi, Babak~Ehteshami Bejnordi, Arnaud Arindra~Adiyoso
  Setio, Francesco Ciompi, Mohsen Ghafoorian, Jeroen~Awm Van Der~Laak, Bram
  Van~Ginneken, and Clara~I S{\'a}nchez.
\newblock A survey on deep learning in medical image analysis.
\newblock {\em Medical image analysis}, 42:60--88, 2017.

\bibitem{long2015fully}
Jonathan Long, Evan Shelhamer, and Trevor Darrell.
\newblock Fully convolutional networks for semantic segmentation.
\newblock In {\em Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pages 3431--3440, 2015.

\bibitem{DBLP:journals/corr/MiyashitaLM16}
Daisuke Miyashita, Edward~H. Lee, and Boris Murmann.
\newblock Convolutional neural networks using logarithmic data representation.
\newblock {\em CoRR}, abs/1603.01025, 2016.

\bibitem{newell2016stacked}
Alejandro Newell, Kaiyu Yang, and Jia Deng.
\newblock Stacked hourglass networks for human pose estimation.
\newblock In {\em European Conference on Computer Vision}, pages 483--499.
  Springer, 2016.

\bibitem{noh2015learning}
Hyeonwoo Noh, Seunghoon Hong, and Bohyung Han.
\newblock Learning deconvolution network for semantic segmentation.
\newblock In {\em Proceedings of the IEEE international conference on computer
  vision}, pages 1520--1528, 2015.

\bibitem{DBLP:journals/corr/abs-1710-01269}
Christian~S. Perone, Evan Calabrese, and Julien Cohen{-}Adad.
\newblock Spinal cord gray matter segmentation using deep dilated convolutions.
\newblock {\em CoRR}, abs/1710.01269, 2017.

\bibitem{pham2000current}
Dzung~L Pham, Chenyang Xu, and Jerry~L Prince.
\newblock Current methods in medical image segmentation.
\newblock {\em Annual review of biomedical engineering}, 2(1):315--337, 2000.

\bibitem{DBLP:journals/corr/abs-1802-05668}
Antonio Polino, Razvan Pascanu, and Dan Alistarh.
\newblock Model compression via distillation and quantization.
\newblock {\em CoRR}, abs/1802.05668, 2018.

\bibitem{DBLP:journals/corr/RastegariORF16}
Mohammad Rastegari, Vicente Ordonez, Joseph Redmon, and Ali Farhadi.
\newblock Xnor-net: Imagenet classification using binary convolutional neural
  networks.
\newblock {\em CoRR}, abs/1603.05279, 2016.

\bibitem{ronneberger2015u}
Olaf Ronneberger, Philipp Fischer, and Thomas Brox.
\newblock U-net: Convolutional networks for biomedical image segmentation.
\newblock In {\em International Conference on Medical image computing and
  computer-assisted intervention}, pages 234--241. Springer, 2015.

\bibitem{shen2017deep}
Dinggang Shen, Guorong Wu, and Heung-Il Suk.
\newblock Deep learning in medical image analysis.
\newblock {\em Annual review of biomedical engineering}, 19:221--248, 2017.

\bibitem{DBLP:journals/corr/ShinBS17}
S.~{Shin}, Y.~{Boo}, and W.~{Sung}.
\newblock Fixed-point optimization of deep neural networks with adaptive step
  size retraining.
\newblock In {\em 2017 IEEE International Conference on Acoustics, Speech and
  Signal Processing (ICASSP)}, pages 1203--1207, March 2017.

\bibitem{TangAndKwan}
Chuan~Zhang Tang and Hon~Keung Kwan.
\newblock Multilayer feedforward neural networks with single powers-of-two
  weights.
\newblock {\em IEEE Transactions on Signal Processing,}, 41(8):, 1993.

\bibitem{Tang2017HowTT}
Wei Tang, Gang Hua, and Liang Wang.
\newblock How to train a compact binary neural network with high accuracy?
\newblock In {\em AAAI}, 2017.

\bibitem{DBLP:journals/corr/WenZLZFZY16}
He~Wen, Shuchang Zhou, Zhe Liang, Yuxiang Zhang, Dieqiao Feng, Xinyu Zhou, and
  Cong Yao.
\newblock Training bit fully convolutional network for fast semantic
  segmentation.
\newblock {\em CoRR}, abs/1612.00212, 2016.

\bibitem{DBLP:journals/corr/abs-1802-04680}
Shuang Wu, Guoqi Li, Feng Chen, and Luping Shi.
\newblock Training and inference with integers in deep neural networks.
\newblock {\em CoRR}, abs/1802.04680, 2018.

\bibitem{DBLP:journals/corr/abs-1803-04907}
Xiaowei Xu, Qing Lu, Yu~Hu, Lin Yang, Xiaobo~Sharon Hu, Danny~Ziyi Chen, and
  Yiyu Shi.
\newblock Quantization of fully convolutional networks for accurate biomedical
  image segmentation.
\newblock {\em CVPR}, pages 8300--8308, 2018.

\bibitem{xu2018quantization}
Xiaowei Xu, Qing Lu, Lin Yang, Sharon Hu, Danny Chen, Yu~Hu, and Yiyu Shi.
\newblock Quantization of fully convolutional networks for accurate biomedical
  image segmentation.
\newblock {\em Preprint at https://arxiv. org/abs/1803.04907}, 2018.

\bibitem{DBLP:journals/corr/ZhouYGXC17}
Aojun Zhou, Anbang Yao, Yiwen Guo, Lin Xu, and Yurong Chen.
\newblock Incremental network quantization: Towards lossless cnns with
  low-precision weights.
\newblock {\em CoRR}, abs/1702.03044, 2017.

\bibitem{DBLP:journals/corr/ZhouNZWWZ16}
Shuchang Zhou, Zekun Ni, Xinyu Zhou, He~Wen, Yuxin Wu, and Yuheng Zou.
\newblock Dorefa-net: Training low bitwidth convolutional neural networks with low bitwidth gradients.
\newblock {\em CoRR}, abs/1606.06160, 2016.

\bibitem{10.1371/journal.pbio.1000502}
Albert Cardona, Stephan Saalfeld, Stephan Preibisch, Benjamin Schmid , Anchi Cheng , Jim Pulokas, Pavel Tomancak, Volker Hartenstein.
\newblock An Integrated Micro- and Macroarchitectural Analysis of the Drosophila Brain by Computer-Assisted Serial Section Electron Microscopy.
\newblock {\em PLOS Biology}, pages 1-17, 2010.
\end{thebibliography}

